Meta-SAC: Auto-tune the Entropy Temperature of Soft Actor-Critic via Metagradient

Exploration-exploitation dilemma has long been a crucial issue in reinforcement learning. In this paper, we propose a new approach to automatically balance between these two. Our method is built upon the Soft Actor-Critic (SAC) algorithm, which uses an "entropy temperature" that balances the original task reward and the policy entropy, and hence controls the trade-off between exploitation and exploration. It is empirically shown that SAC is very sensitive to this hyperparameter, and the follow-up work (SAC-v2), which uses constrained optimization for automatic adjustment, has some limitations. The core of our method, namely Meta-SAC, is to use metagradient along with a novel meta objective to automatically tune the entropy temperature in SAC. We show that Meta-SAC achieves promising performances on several of the Mujoco benchmarking tasks, and outperforms SAC-v2 over 10% in one of the most challenging tasks, humanoid-v2.

==> 4measure.tex <==
% Drafted by Tianwei
\section{Exploration Measures for Evaluation}
% \tw{I change the term metrics to measures because in math, metric is a distance function, which may be confusing. Measure is derived from information theory, with strong connection with entropy.}

RL agents aim to coordinate the relationship between exploration and exploitation. However, in many RL algorithms these two are entangled and it's hard to distinguish which one prevails over the other during the training stage. Though \textit{exploitation} could be well measured by (testing) returns, i.e. a typical \textbf{exploitation measure}, exploration remains mystified, thus motivating us to propose the information measures of \textit{exploration}, i.e. \textbf{exploration measures}. 
To go further, off-policy RL algorithms have different policies for exploration and exploitation, named \textit{behavior} policies and \textit{test} policies, respectively.\footnote{In SAC, behavior policy samples actions from predicted distribution while test policy uses expected actions; in DDPG, behavior policy injected noise to predicted action while test policy directly uses predicted actions.} Thus for fair comparison, we need to compute exploration and exploitation measures induced by behavior and target policies separately. % Extrapolation Error

Now we aim to examine the exploration ability of behavior policies in RL algorithms. Traditionally, exploration is measured in state space, usually in a form of functions of state visitation frequencies. Additionally, we can view exploration from trajectory (state-action visitation) perspective, since agents keep rolling out trajectories during exploration and learning. Hence, we propose two information measures of exploration for evaluation in state space and trajectory space, respectively, for \textit{any} behavior policy.

\subsection{Entropy of State Marginal Distribution}

For exploration in state space, one of intrinsic measure is the entropy of distribution over (visited) state space \cite{hazan2019provably}, reaching the maximum when it's a uniform distribution. Thus naturally, \textit{entropy}, the measure of uncertainty in a distribution, could be introduced into evaluation of exploration ability. As the realization of state distribution, we take the definition of (non-discounted) state marginal distribution \cite{lee2019efficient} $\rho^\pi(\sv)$\footnote{In this section and corresponding appendix, $\pi$ refers to the behavior policy in an RL algorithm.} in a finite horizon $T$.\footnote{We don't adopt the discounted (stationary) state marginal distribution \cite{silver2014deterministic} because our task is episodic with finite horizon and the measures will be approximated by collection of visited states.}

\begin{align}
\label{eq:state_marg}
\rho^\pi(\sv)\defeq 
\Eb{\substack{\sv_0\sim p(\sv_0)\\\av_t\sim \pi\\\sv_{t+1}\sim \env}}
{\frac{1}{T}\sum_{t=0}^{T-1} \mathbbm{1}(\sv_t=\sv)}
\end{align}

Based on the state density in Eq \ref{eq:state_marg}, we can approximate its entropy $\hat{\mathcal{H}}_{\sv}^\pi$ since it's intractable to have a closed form. The approximation method will be introduced in section \ref{sec: marg}.

\subsection{Empirical Entropy Rate of State-Action Trajectory Distribution}
\label{sec: traj_ent}
% \tw{Non-stationary process, not gauranteed to converge. Given \textit{deterministic} transition in Mujoco, State-Action Trajectory Entropy Rate is proved to be exactly $\frac1T\sum_{t=1}^T\Eb{\sv_t\sim \rho_t^\pi(\sv_t)}{\mathcal H(\pi(\cdot|\sv_t)}$ lmao. Using chain rule. TODO.}

Now we investigate the exploration from a novel perspective -- in state-action trajectory space. Let $\xv_t = (\sv_t, \av_t)$ be state-action pair at time $t$, then trajectory of horizon $T$ can be expressed as $\tau = (\xv_0, \xv_1, \dots, \xv_{T-1})$, which is a finite discrete-time Markov chain. For a Markov chain, we normally estimate its Shannon entropy rate \cite{cover2012elements} $\ent (\xv)=\lim_{T\to \infty} \ent (\xv_0,\dots, \xv_{T-1})/T$ instead of entropy, which shows entropy growth w.r.t. time. Since the trajectory $\tau$ is finite\footnote{In our setting, MDP is not stationary and its state space is non-countable, so its entropy rate cannot be guaranteed to converge in theory.}, we can approximate its \textit{empirical entropy rate} by $\ent (\tau)=\ent (\xv_0,\dots, \xv_{T-1})/T$ \cite{ekroot1993entropy, han2018entropy}. By derivation (Appendix \ref{sec:traj_proof}), we show the empirical entropy rate:

\begin{equation}
\label{eq:traj_ent_rate}
\begin{split}
\ent^\pi_\tau &\defeq \frac{1}{T} \ent(\xv_0,\dots, \xv_{T-1})\\
&= \frac1T \Bigg(\ent[p(\sv_0)] + \Eb{\sv_0\sim p(\sv_0)}{\ent[\pi(\cdot|\sv_0)]} + \\
& ~~~~ \sum_{t=1}^{T-1} \ent[p(\cdot|\sv_{t-1},\av_{t-1})] + \Eb{\sv_t\sim p}{\ent[\pi(\cdot|\sv_t)]} \Bigg)
\end{split}
\end{equation}

Generally, we don't have access to the transition probability $p(\sv_t|\sv_{t-1},\av_{t-1})$ and our setting is model-free RL, thus the entropy rate seems intractable. However, under the assumption of \textit{deterministic} dynamics\footnote{Our experiment environment Mujoco \cite{todorov2012mujoco} is designed to have deterministic transition except stochastic initial state.}, the entropy rate can be simplified as:

\begin{equation}
\label{eq:traj_ent_rate_det}
\begin{split}
\ent^\pi_\tau = \frac1T \left(\ent[p(\sv_0)] + \Eb{\sv_0}{\ent[\pi(\cdot|\sv_0)]} + \sum_{t=1}^{T-1} \ent[\pi(\cdot|\sv_t)] \right)
\end{split}
\end{equation}

Given deterministic transition, it's worthwhile to note that this measure has strong connection with Soft Actor-Critic (Eq \ref{eq:sac}). Actually, SAC's entropy term can be transformed as $T\ent^\pi_\tau - \ent[p(\sv_0)]$. Thus trajectory entropy rate $\ent^\pi_\tau$ can be viewed as the time-average of action entropies along trajectory, reaching its maximum when behavior policy is uniformly random (see derivation in Appendix \ref{sec:traj_max_ent}). 

\tw{to be frank, this is trivial under deterministic environment}

\subsection{Derivation}

\subsubsection{State Marginal Distribution w.r.t. Time}
\tw{should we add this?}

The trajectory distribution over $\tau=(\sv_0,\av_0,\sv_1,...,\sv_{T-1})$ following a
a policy $\pi(a|s)$ within a fixed horizon $T$ can be given by:

\begin{align}
\label{eq:traj_dist}
u^{\pi}(\tau) = p(\sv_0)\prod_{t=0}^{T-2} \left(\pi(\av_t|\sv_t)p(\sv_{t+1}|\sv_t,\av_t)\right)
\end{align}

We can marginalize the trajectory distribution to obtain it.
\begin{align}
\begin{split}
\rho_t^\pi(\sv_t) &= \int u^\pi(\sv_0,\av_0,\sv_1,...,\sv_t) d\sv_0\,d\av_0\dots d\av_{t-1}\\
&= \int p(\sv_0)\prod_{i=0}^{t-1} \left(\pi(\av_i|\sv_i)p(\sv_{i+1}|\sv_i,\av_i)\right) d\sv_0\,d\av_0\dots d\av_{t-1}
\end{split}
\end{align}

\subsubsection{Derivation of Trajectory Empirical Entropy Rate $\mathcal H^\pi_\tau$}
\label{sec:traj_proof}

According to definition in the main paper, we use chain rule of joint entropy and Markov property to derive as follows:

\begin{equation}
\begin{split}
\ent^\pi_\tau &\defeq \frac{1}{T} \ent(\xv_0,\dots, \xv_{T-1})\\
&= \frac1T \left(\ent(\xv_0) + \sum_{t=1}^{T-1} \ent(\xv_{t}|\xv_{t-1},\dots,\xv_0) \right)\\
&= \frac1T \left(\ent(\xv_0) + \sum_{t=1}^{T-1} \ent(\xv_{t}|\xv_{t-1}) \right)\\
&= \frac1T \Bigg(\Eb{\substack{\sv_0 \sim p(\sv_0)\\ \av_0\sim \pi}}{-\log p(\sv_0)\pi(\av_0|\sv_0)} + \\
& ~~~~ \sum_{t=1}^{T-1} \Eb{\substack{\sv_t \sim p\\ \av_t\sim \pi}}{-\log p(\sv_t|\sv_{t-1},\av_{t-1})\pi(\av_t|\sv_t)} \Bigg)\\
&= \frac1T \Bigg(\ent(p(\sv_0)) + \Eb{\sv_0\sim p(\sv_0)}{\ent(\pi(\cdot|\sv_0))} + \\
& ~~~~ \sum_{t=1}^{T-1} \ent(p(\cdot|\sv_{t-1},\av_{t-1})) + \Eb{\sv_t\sim p}{\ent(\pi(\cdot|\sv_t))} \Bigg)
\end{split}
\end{equation}

\subsubsection{Entropy Term in SAC objective }
\label{sec:traj_max_ent}

SAC objective is derived from MaxEnt RL framework \cite{levine2018reinforcement}, which is from negative KL divergence over a fixed horizon between the trajectory distribution of \textit{optimal} policy $\pi$ and that of uniformly random policy $\pi'=1/|\mathcal{A}|$ given fixed dynamics. Now consider $\pi$ is \textit{any} policy, then we can derive entropy term in SAC objective by:  

\begin{equation}
\label{eq:traj_dev}
\begin{split}
-&D_{KL}(u^{\pi}(\tau)||u^{\pi'}(\tau)) \\
&= \Eb{\tau\sim u^{\pi}(\tau)}{\log \frac{u^{\pi'}(\tau)}{u^{\pi}(\tau)}}\\
&= \Eb{\tau\sim u^{\pi}(\tau)}
{\log \frac
{\cancel{p(\sv_1)} \prod_{t=0}^{T-1} \cancel{p(\sv_{t+1}|\sv_t,\av_t)}\pi'(\av_t|\sv_t)}
{\cancel{p(\sv_1)}\prod_{t=0}^{T-1} \cancel{p(\sv_{t+1}|\sv_t,\av_t)}\pi(\av_t|\sv_t)}}\\
&= \Eb{\tau\sim u^{\pi}(\tau)}{-\sum_{t=1}^T \log\pi(\av_t|\sv_t)} - T\log|\mathcal A|\\
&= \sum_{t=0}^{T-1}\Eb{\substack{\sv_t\sim \rho_t^\pi(\sv_t)\\\av_t\sim \pi(\av_t|\sv_t)}}{ -\log\pi(\av_t|\sv_t)} - T\log|\mathcal A|\\
&= \sum_{t=0}^{T-1}\Eb{\sv_t\sim \rho_t^\pi(\sv_t)}{\mathcal H(\pi(\cdot|\sv_t)} - T\log|\mathcal A|
\end{split}
\end{equation}

, where $\rho_t^\pi(\sv)$ is the state marginal distribution w.r.t. time $t$ for the target policy $\pi$. The first term is exactly entropy term in SAC objective.

\subsubsection{Approximation of Trajectory Empirical Entropy Rate $\hat{\mathcal H}^\pi_\tau$}
\label{sec: approx_traj}
We can approximate $\mathcal H^\pi_\tau$ based on Eq \ref{eq:traj_ent_rate_det} by sampling trajectories induced by the policy. Note that $\ent^\pi_\tau$ contains a \textit{constant} term of initiate state entropy given an environment, thus we can ignore this term for estimator $\hat{\mathcal H}^\pi_\tau$. Let $N_t$ be the number of sampled states at timestamp $t$. Then $\hat{\mathcal H}^\pi_\tau$ can derived as:

\begin{equation}
\label{eq:traj_mc}
\begin{split}
\hat{\mathcal H}^\pi_\tau &= \frac1T\sum_{t=0}^{T-1}\frac{1}{N_t}\left(\sum_{i=1}^{N_t}\ent[\pi(\cdot|\sv_t^{(i)})]\right)
\end{split}
\end{equation}
, where $\sv_t^{(i)}$ is the $i$-th sample of states at time $t$.

We can simplify the estimation by assuming that all the sampled trajectories has a horizon of exact $T$\footnote{which is often the case in mujoco environments of reaching the maximum horizon $T=1000$ for a moderate policy}, i.e. $N_t=N_s$ for any $t=0,1,...,T-1$. The total number of visited states is now $N=\sum_{t=0}^{T-1} N_t=T N_s$. Under this assumption, we have a practical approximation:

\begin{equation}
\label{eq:traj_mcT}
\begin{split}
\hat{\mathcal H}^\pi_\tau &\approx\frac{1}{TN_s}\sum_{t=1}^T\left(\sum_{i=1}^{N_s}\mathcal H[\pi(\cdot|\sv_t^{(i)})]\right)\\
&= \frac{1}{TN_s}\sum_{j=1}^{TN_s}\mathcal H[\pi(\cdot|\sv^{(j)})]\\
&= \frac{1}{N}\sum_{j=1}^{N}\mathcal H[\pi(\cdot|\sv^{(j)})]\\
\end{split}
\end{equation}
, where $\sv^{(j)}$ is the $j$-th sampled state.


\subsection{Exploration Evaluation}
% Drafted by Tianwei

There are several key questions: 
\begin{itemize}
    \item To what extent does an RL agent explore in an environment during training stage? How does the exploration evolve w.r.t. training iterations?
    \item What's the relationship between exploration and exploitation during training? Does an optimal stochastic agent behave in a way that first explores broadly with high entropy to absorb environment information, and then quickly narrows its visited state space and become deterministic? \tw{I expect to name it as intelligent/efficient exploration.}
\end{itemize}

Empirically, we can answer these questions by obtaining the curves of exploration measures (defined above) and the typical exploitation measure (a.k.a returns) w.r.t. training iterations, and compare them via correlation analysis across different RL algorithms.


Humanoid-v2 is one of the most challenging continuous control environments solvable by state-of-the-art RL algorithms \cite{salimans2017evolution}, with high dimension of state space (376) and action space (17). Thus it's crucial to take this as an example to compare different RL algorithms via our exploration measures.

\subsubsection{State Marginal Entropy}
\label{sec: marg}

For the approximation of State Marginal Entropy $\hat{\mathcal{H}}_{\sv}^\pi$ given a policy (snapshot) $\pi$, we need to collect the visited states, the support of State Marginal distribution. In off-policy RL, the visited state collection is also known as replay buffer. 

Due to the high dimension in state space and huge number of samples, we have to reduce its dimension by incremental PCA \cite{scikit-learn, ross2008incremental}, and choose the reduced dimension of $15$ by the threshold of $99\%$ in the explained variance ratio over components.
\tw{I don't find papers on PCA's information loss on entropy.}

A simple method to approximate entropy given low-dimension samples is firstly (1) Kernel Density Esimation and then (2) plug-in entropy estimator given the approximated density. However, this causes unbearable information loss and time cost. We circumvent density esimation by employing a non-parametric Kozachenko-Leonenko (KL) entropy estimator \cite{kozachenko1987sample, kraskov2004estimating}. Suggested by \cite{ver2000non}, we choose $k=3$ as k-nearest neighbor in KL estimator, which has low bias bound shown in \cite{singh2016analysis}.

\tw{exp}

\subsubsection{Trajectory Empirical Entropy Rate}
Next, we evaluate the exploration of our policy using the measure of trajectory entropy rate defined in Eq \ref{eq:traj_ent_rate_det} since Mujoco dynamics are deterministic. To approximate this measure (derived in Appendix \ref{sec: approx_traj}), we sample trajectories to compute:
\begin{equation}
\begin{split}
\hat{\mathcal H}^\pi_\tau &\approx \frac{1}{N}\sum_{j=1}^{N}\mathcal H[\pi(\cdot|\sv^{(j)})]\\
\end{split}
\end{equation}
, where $N$ is the number of visited states and $\sv^{(j)}$ is the $j$-th sampled state.

\tw{exp}


\subsubsection{Discussion}
\tw{ Personally, I think this subsection is essential to our empirical claim: (1) use our measures to evaluate and compare our method with others. (2) explain the relationship between two measures by some algorithms, and also in turn indicating the intrinsic property of these algorithms. EE can be seen as two time series, RL final goal is to make Exploit time series quickly reach higher value. Then how about Explore time series?}

Expected Goal: 

SAC, a Max Action/Trajectory Entropy (showed in sec 4) method. DDPG/TD3, deterministic policy. Our method, based on SAC with deterministic (in action space) meta objective.

In humanoid, SAC enjoys \textit{consistently} highest Traj Entropy than our methods and DDPG (zero), aligned with objective.

\textbf{However, max action/traj entropy is only one kind of exploration measures, which does not \textit{ensure} exploration in state space.}\cite{islam2019marginalized} For example, max act/traj entropy policy reduces to random walk with low entropy in state space given sparse rewards (may cite). Empirically, our method has greatest state marginal entropy in the earlier training stage, which means we explores much faster and broader than SAC/DDPG in state space.

Synthesized with exploitation measure, our method greatly outperforms SAC/DDPG in humanoid, suggesting that \textit{in our setting} faster and broader exploration in state space \textbf{may be a stronger indicator} than in traj space for better exploitation by means of our method (a hybrid one of stochastic and deterministic policies). 



\textbf{Exploration and State Distribution}. Among exploration RL algorithms, some of them define various kinds of marginalized state distributions and approximate entropies of them as regularization for better exploration.
\cite{hazan2019provably} approximated discounted state distribution by discretization in continuous state space and proposed its several quantities such as entropy, for training an exploration policy solely. 
\cite{lee2019efficient} proposes state non-discounted marginal distribution and use a parametric density model to estimate its entropy, also for only training a exploration policy.
\cite{vezzani2019learning, islam2019off} train VAEs \cite{kingma2013auto} to estimate log density of latent state distribution for entropy regularization.
\cite{islam2019marginalized} approximates discounted state marginal entropy by variational method and leverages it as regularization in policy gradient.

One of our exploration measure is (non-discounted) state marginal entropy, however we don't explicitly regularize state marginal entropy in our training objective, instead we examine this measure for evaluation, which lacks attention in RL community.
\cite{vezzani2019learning, shyam2019model} plot trajectories of visited states in 2D environments to visualize exploration and action entropy.
\cite{xu2018learning} plots the state visitation density contours after dimension reduction from a 11-dim space by t-SNE \cite{maaten2008visualizing} to visualize difference in exploration between teacher and student policy. In comparison, our method builds a tractable entropy estimator from high-dimensional space distribution and provides detailed quantitative analysis on exploration. Moreover, we also derived another measure of trajectory entropy rate to evaluate exploration, which has been little investigated.

